Simulating the effect of the Sgr A* accretion flow on the appearance of G2 after pericenter

We study the dynamical interaction of the G2 cloud with the accretion flow around Sgr A* by means of three-dimensional, hydrodynamic simulations. We show the effects of the rotating accretion flow on the evolution of G2 by projecting the cloud density onto the plane of the sky, and extracting position-velocity diagrams. We study a number of possible orientations of the cloud orbit with respect to the disk. We find that once the center of mass of the cloud has crossed the pericenter, the differences between models becomes significant. Models with the cloud counter-rotating with respect to the disk are expected to reach higher blue-shifted line of sight velocities. The spatial extent of the emission depends strongly on the cloud-to-disk inclination angle. Future imaging and spectroscopy of G2 emission will shed light both on the structure of the Sgr A* disk and on the properties of the cloud.

==> G2 Final/figurelist <==
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/counter20124.png}}\\\vspace{-1cm}
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/counter20133gilplusdisk.png}}
\subfigure{\includegraphics[height=.2\textwidth,]{figures/testparticles20134posvel.png}} \\
&\subfigure{\includegraphics[height=.2\textwidth,]{figures/gillessen20133posvelco.png}}\\
&\subfigure{\includegraphics[height=.2\textwidth,]{figures/gillessen20133posvelcounter.png}}\\
&\subfigure{\includegraphics[width=.3\textwidth,]{figures/gillessenposvelcolorbar.png}}
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/co2012density.png}} \\\vspace{-1cm}
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/co2012temp.png}}
	\subfigure{\includegraphics[height=.26\textwidth,]{figures/co20134density.png}} &
	%\subfigure{\includegraphics[height=.26\textwidth]{figures/co20139density.png}} 
	\subfigure{\includegraphics[height=.26\textwidth]{figures/co201425density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth,]{figures/co20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/co20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/counter20146density.png}} &
        \subfigure{\includegraphics[height=.26\textwidth]{figures/300M20146density.png}} 
	\subfigure{\includegraphics[height=.26\textwidth]{figures/coinc20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/counterinc20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/oneM20146density.png}} 
 \subfigure{\includegraphics[width=.45\textwidth,]{figures/co20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counter20146_3D.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coinc20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterinc20146_3D.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coincref20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterincref20146_3D.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/oneM20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/300M20146_3D.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/co20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/counter20146skydensityrhosq.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/coinc20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/counterinc20146skydensityrhosq.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/coincref20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/counterincref20146skydensityrhosq.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/oneM20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/300M20146skydensityrhosq.png}} \\
    &\multicolumn{2}{c}{\subfigure{\includegraphics[width=0.4\textwidth]{figures/skydensitycolorbar.png}}} \\
 \subfigure{\includegraphics[width=.45\textwidth,]{figures/co20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counter20146LOSvelocity.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coinc20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterinc20146LOSvelocity.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coincref20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterincref20146LOSvelocity.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/oneM20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/300M20146LOSvelocity.png}} \\
	 &\multicolumn{2}{c}{\subfigure{\includegraphics[width=0.4\textwidth]{figures/skyvelocitycolorbar.png}}} \\
	\subfigure{\includegraphics[width=.3\textwidth,]{figures/co20134posvelrhosq.png}} \\
%	\subfigure{\includegraphics[width=.3\textwidth,]{figures/co20139posvel.png}} \\
	\subfigure{\includegraphics[width=.3\textwidth]{figures/co201425posvelrhosq.png}} \\
	\subfigure{\includegraphics[width=.3\textwidth]{figures/co20146posvelrhosq.png}} \\
	&\subfigure{\includegraphics[width=.3\textwidth]{figures/posvelcolorbar.png}} \\
	\begin{sideways}\large pos(mas)\end{sideways} &\subfigure{\includegraphics[width=.4\textwidth]{figures/co20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/counter20146posvelrhosq.png}} \\
	\begin{sideways}\large pos(mas)\end{sideways}&\subfigure{\includegraphics[width=.4\textwidth]{figures/coinc20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/counterinc20146posvelrhosq.png}} \\
	\begin{sideways}\large pos(mas)\end{sideways}&\subfigure{\includegraphics[width=.4\textwidth]{figures/coincref20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/counterincref20146posvelrhosq.png}} \\
	 \begin{sideways}\large pos(mas)\end{sideways}&\subfigure{\includegraphics[width=.4\textwidth]{figures/oneM20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/300M20146posvelrhosq.png}} 	\\
	&\multicolumn{2}{c}{\subfigure{\includegraphics[width = 0.4\textwidth]{figures/posvelcolorbar.png}} } 
  	\subfigure{\includegraphics[height=.2\textwidth,]{figures/cocounterpvcontourrhosq.png}} & 
	\subfigure{\includegraphics[height=.2\textwidth,]{figures/oneM300Mpvcontourrhosq.png}} \\
	\subfigure{\includegraphics[height=.2\textwidth,]{figures/cocounterincpvcontourrhosq.png}}  &
	\subfigure{\includegraphics[height=.2\textwidth,]{figures/cocounterincrefpvcontourrhosq.png}}  \\


==> figurelist <==
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/counter20124.png}}\\\vspace{-1cm}
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/counter20133gilplusdisk.png}}
\subfigure{\includegraphics[height=.2\textwidth,]{figures/testparticles20134posvel.png}} \\
&\subfigure{\includegraphics[height=.2\textwidth,]{figures/gillessen20133posvelco.png}}\\
&\subfigure{\includegraphics[height=.2\textwidth,]{figures/gillessen20133posvelcounter.png}}\\
&\subfigure{\includegraphics[width=.3\textwidth,]{figures/gillessenposvelcolorbar.png}}
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/co2012density.png}} \\\vspace{-1cm}
\subfigure{\includegraphics[width=.9\columnwidth,]{figures/co2012temp.png}}
	\subfigure{\includegraphics[height=.26\textwidth,]{figures/co20134density.png}} &
	%\subfigure{\includegraphics[height=.26\textwidth]{figures/co20139density.png}} 
	\subfigure{\includegraphics[height=.26\textwidth]{figures/co201425density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth,]{figures/co20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/co20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/counter20146density.png}} &
        \subfigure{\includegraphics[height=.26\textwidth]{figures/300M20146density.png}} 
	\subfigure{\includegraphics[height=.26\textwidth]{figures/coinc20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/counterinc20146density.png}} &
	\subfigure{\includegraphics[height=.26\textwidth]{figures/oneM20146density.png}} 
 \subfigure{\includegraphics[width=.45\textwidth,]{figures/co20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counter20146_3D.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coinc20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterinc20146_3D.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coincref20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterincref20146_3D.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/oneM20146_3D.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/300M20146_3D.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/co20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/counter20146skydensityrhosq.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/coinc20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/counterinc20146skydensityrhosq.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/coincref20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/counterincref20146skydensityrhosq.png}} \\
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/oneM20146skydensityrhosq.png}} &
    \subfigure{\includegraphics[width=.45\textwidth,]{figures/300M20146skydensityrhosq.png}} \\
    &\multicolumn{2}{c}{\subfigure{\includegraphics[width=0.4\textwidth]{figures/skydensitycolorbar.png}}} \\
 \subfigure{\includegraphics[width=.45\textwidth,]{figures/co20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counter20146LOSvelocity.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coinc20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterinc20146LOSvelocity.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/coincref20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/counterincref20146LOSvelocity.png}} \\
\subfigure{\includegraphics[width=.45\textwidth,]{figures/oneM20146LOSvelocity.png}} &
\subfigure{\includegraphics[width=.45\textwidth,]{figures/300M20146LOSvelocity.png}} \\
	 &\multicolumn{2}{c}{\subfigure{\includegraphics[width=0.4\textwidth]{figures/skyvelocitycolorbar.png}}} \\
	\subfigure{\includegraphics[width=.3\textwidth,]{figures/co20134posvelrhosq.png}} \\
%	\subfigure{\includegraphics[width=.3\textwidth,]{figures/co20139posvel.png}} \\
	\subfigure{\includegraphics[width=.3\textwidth]{figures/co201425posvelrhosq.png}} \\
	\subfigure{\includegraphics[width=.3\textwidth]{figures/co20146posvelrhosq.png}} \\
	&\subfigure{\includegraphics[width=.3\textwidth]{figures/posvelcolorbar.png}} \\
	\begin{sideways}\large pos(mas)\end{sideways} &\subfigure{\includegraphics[width=.4\textwidth]{figures/co20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/counter20146posvelrhosq.png}} \\
	\begin{sideways}\large pos(mas)\end{sideways}&\subfigure{\includegraphics[width=.4\textwidth]{figures/coinc20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/counterinc20146posvelrhosq.png}} \\
	\begin{sideways}\large pos(mas)\end{sideways}&\subfigure{\includegraphics[width=.4\textwidth]{figures/coincref20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/counterincref20146posvelrhosq.png}} \\
	 \begin{sideways}\large pos(mas)\end{sideways}&\subfigure{\includegraphics[width=.4\textwidth]{figures/oneM20146posvelrhosq.png}} &
	\subfigure{\includegraphics[width=.4\textwidth]{figures/300M20146posvelrhosq.png}} 	\\
	&\multicolumn{2}{c}{\subfigure{\includegraphics[width = 0.4\textwidth]{figures/posvelcolorbar.png}} } 
  	\subfigure{\includegraphics[height=.2\textwidth,]{figures/cocounterpvcontourrhosq.png}} & 
	\subfigure{\includegraphics[height=.2\textwidth,]{figures/oneM300Mpvcontourrhosq.png}} \\
	\subfigure{\includegraphics[height=.2\textwidth,]{figures/cocounterincpvcontourrhosq.png}}  &
	\subfigure{\includegraphics[height=.2\textwidth,]{figures/cocounterincrefpvcontourrhosq.png}}  \\

